StyleGAN-NADA: CLIP-Guided Domain Adaptation of Image Generators

Can a generative model be trained to produce images from a specific domain, guided by a text prompt only, without seeing any image? In other words: can an image generator be trained "blindly"? Leveraging the semantic power of large scale Contrastive-Language-Image-Pre-training (CLIP) models, we present a text-driven method that allows shifting a generative model to new domains, without having to collect even a single image. We show that through natural language prompts and a few minutes of training, our method can adapt a generator across a multitude of domains characterized by diverse styles and shapes. Notably, many of these modifications would be difficult or outright impossible to reach with existing methods. We conduct an extensive set of experiments and comparisons across a wide range of domains. These demonstrate the effectiveness of our approach and show that our shifted models maintain the latent-space properties that make generative models appealing for downstream tasks.

==> intro.tex <==
\section{Introduction}
\label{sec:intro}

The unprecedented ability of GANs \cite{goodfellow2014generative} to capture and model distributions through a semantically-rich latent space has revolutionized countless fields. These range from unconditional image synthesis \cite{karras2020analyzing}, through editing, image-to-image translation, super resolution \cite{ledig2017photo}, restoration \cite{yang2021gan}, animation, and more recently even discriminative tasks such as classification and regression \cite{xu2021generative}. \gal{In the ML community, we usually try to get to the point faster. E.g. cut praises to GAN get to the main point of the paper, already of 1st par. }

\input{resources/figures/teaser}

However, the applicability of GAN-based methods is often constrained by a critical requirement - modern GANs require tens of thousands \cite{karras2019style} and even millions \cite{brock2018large} of images to properly converge. Such image collections are often prohibitively difficult to acquire, owing to quality, privacy and copyright constraints \cite{Karras2020ada}. Indeed, in many cases (paintings by specific artists, extinct animals), there may not even exist sufficient data to train a GAN.

Imagine a world where we could do away with such requirements and train a GAN to synthesize a variety of subjects from \textit{any} class - without providing it with a single image of the target domain. With such zero-shot training, an artist could use GANs to edit \textit{any} image, their creativity unconstrained by the availability of pre-trained models \gal{of samples? We didnt talk about pre-trained models yet}. In such a world, a practitioner of machine learning could simply synthesize a complete dataset from scratch and use it train models for downstream tasks -- no matter their domain. 

In this work, we take the first steps towards realizing such a world. 
We follow the recently introduced StyleCLIP method \gal{I would reorder slightly: spend a par' about StyleCLIP, then state the limitation and our solution} in combining the power of Contrastive Language-Image Pre-training (CLIP) models with a style-based generator to enable intuitive \textit{text-based} semantic image manipulations. However, while StyleCLIP enables text-based manipulations of images, it does so by discovering meaningful directions within the latent space of the GAN. As such, it can only induce changes that lie \textit{within} the domain of a pre-trained generator. In contrast, we employ CLIP  to guide a \textbf{translation of the generator itself}. We modify the generator's weights and shift it \textit{outside} of its original source domain and towards \textit{new domains}. \dc{I would like to have here the term "out-of-domain"}

To leverage CLIP effectively for text-guided training, we propose a new dual-generator training approach. These generators are \textit{intertwined}, sharing a joint latent space and a mapping network \rgc{too stylegan specific?}. One generator is kept frozen for the duration of the training - providing us with the context of the source domain across an infinite range of generated identities. The other generator is trained, not to maximize some CLIP-based classification score (a process which leads to adversarial solutions \cite{goodfellow2014explaining}), but rather to \textit{shift} each generated identity, individually, along some textually-prescribed path in CLIP's multi-modal embedding space. 

With such a mechanism, we can already adapt the generator across a wide range of domains. Through a simple text-based interface and a few minutes of training, we can shift the generator across a multitude of styles and shapes, many of which would have been difficult or outright impossible to reach with existing methods.

Even so, we observe that for more drastic shape transformations, additional regularization and stability are required in order to prevent mode collapse before training completes. Following prior approaches, we propose to increase stability in two ways: First, we limit the sub-space of trainable weights. However, contrary to prior methods, we suggest an adaptive approach that utilizes CLIP in order to identify and select the most relevant layers for optimization at each training iteration, and for each target domain. Second, we observe that in most cases, the generator is already capable of producing a mixture of samples from both the source and target domains before quality deteriorates. As such, we can finalize the transition by making use of StyleCLIP's ability to navigate between different modes \textit{within} the domain of a generator. We train a latent-code mapper and utilize it to shift all codes to the regions of the latent space which best match the target domain.


By combining these methods, we can use the flexibility of natural language to affect a truly dazzling array of modifications. These range all the way from high quality toonifications to cross-species adaptation (such as turning dogs to bears and pigs), including imagined domains for which training data does not exist.

We further show that our method maintains the appealing structure of the latent space. Our shifted generator not only inherits the editing capabilities of the original, but it can even re-use any off-the-shelf editing directions and models trained for the original domain.

Finally, we also demonstrate the surprising superiority of our approach to few-shot methods. We show that our method better preserves identities, achieves increased diversity, maintains higher visual quality, and trains at a fraction of the time (\textit{minutes} rather than days) -- and it does so without \textit{any} training data.

Code is available at \href{https://github.com/rinongal/StyleGAN-nada}{github.com/rinongal/StyleGAN-nada}



==> method.tex <==
\input{resources/figures/fig_arch}

\section{Method}
\label{sec:method}


\rev{Our goal is to shift a pre-trained generator from a given source domain to a new target domain, described only through textual prompts, with no images. As a source of supervision, we solely use a pre-trained CLIP model.

This approach entails two main challenges
In order to approach this task, we ask ourselves two key questions: (1) How can we best distill the semantic information encapsulated in CLIP? and (2) How should we regularize the optimization process in order to avoid adversarial solutions or mode collapse? In the following section we outline a training scheme and a set of losses that seek to answer both questions.}

\subsection{Network Architecture}
We begin by outlining the architecture used during our training phase. At the core of our method are two \textit{intertwined} generators, both utilizing the StyleGAN2 \cite{karras2020analyzing} architecture. The generators share a mapping network, and thus the same latent space, such that the same latent code will initially produce the same image in both. We initialize both generators using the weights of a model pre-trained on a single source domain (\eg human faces, dogs, churches or cars). Our goal is to change the domain of one of the paired generators, while keeping the other fixed as a reference. We dub these generators $G_{train}$ and $G_{frozen}$ respectively. 

We guide the change in the trainable generator using a set of CLIP-based losses and a layer-freezing scheme which increases training stability by adaptively determining the most relevant subset of layers to train at each iteration - and freezing the rest. Our training architecture is shown in \cref{fig:arch}. The losses and layer-freezing schemes are detailed below.

\subsection{CLIP-based Guidance}
We rely on a pre-trained CLIP model to serve as the sole source of supervision for our target domain. In order to effectively extract knowledge from CLIP, we utilize three different losses: a global target loss, a local direction loss and an embedding-norm loss.

\paragraph{Global CLIP loss:}
The first and most intuitive of the losses is the global loss described in \cref{eq:global_loss}. Recall that this loss seeks to minimize the CLIP-space cosine distance between the generated images and some given target text.

This loss, however, suffers from a set of shortcomings: First, such a loss sees no benefit from maintaining diversity. Indeed, a mode-collapsed generator which produces the same image regardless of latent code may be the best minimizer for the distance.
Second, it is highly susceptible to adversarial solutions. Without sufficient regularization, the model can opt to fool the classifier (CLIP) by adding appropriate pixel-level perturbations to the image.

These shortcomings make the global loss unsuitable for training the generator. However, we still leverage it in order to adaptively determine which subset of layers to train at each iteration (see \cref{subsec:layer_freezing}).

\rgc{Add clip space visualization}

\paragraph{Directional CLIP loss:} Our second loss is thus designed with the goal of preserving diversity and discouraging extensive image corruption. For this loss, we utilize a pair of images - one generated by the reference (frozen) generator, and another generated by the modified (trainable) generator using the same latent code. Rather than optimizing for better classification (or similarity) score, we draw inspiration from StyleCLIP's global direction approach. We demand that the CLIP-space direction between the embedding of the reference (source) and modified (target) images aligns with the CLIP-space direction between the embeddings of a pair of source and target texts. An illustration of this idea is provided in Fig. \ref{fig:direction}.
\input{resources/figures/direction_loss}
The direction loss is thus given by: 

\begin{equation}
\begin{gathered}
\Delta T = E_{T}\left(t_{target}\right) - E_{T}\left(t_{source}\right)~, \\
\Delta I = E_{I}\left(G_{train}\left(w\right)\right) - E_{I}\left(G_{frozen}\left(w\right)\right)~, \\ 
\mathcal{L}_{direction} = 1 - \frac{\Delta I \cdot \Delta T}{\left|\Delta I\right|\left|\Delta T\right|}~,
\end{gathered}
\end{equation}\label{eq:directional_loss} 
where $E_{I}$ and $E_{T}$ are CLIP's image and text encoders respectively, $G_{frozen}$ and $G_{train}$ are the frozen source generator and the modified trainable generator, and $t_{target}$, $t_{source}$ are the source and target class texts.

Such a loss overcomes the global loss' shortcomings: First, it is adversely affected by mode-collapsed examples. If the target generator only creates a single image, the CLIP-space directions from all sources to this target image will be different. As such, they can't all align with the textual direction. Second, it is harder for the network to converge to adversarial solutions, because it has to engineer perturbations that fool CLIP across an infinite set of different instances. 

%

\subsection{Layer-Freezing}\label{subsec:layer_freezing}

For domain shifts which are predominantly texture-based (\eg photo to sketch) training quickly converges before mode collapse or overfitting occurs. However, more extensive shape modifications require longer training. This in turn destabilizes the network and leads to poor results.

Prior work in the field of few-shot generator domain translation observed that the quality of translated images can be significantly improved by restricting the training to a subset of network weights \cite{mo2020freeze,Robb2020FewShotAO}. 
Intuitively, some layers of the source generator are still useful for generating aspects of the target domain. As such, there is benefit in preserving them. Optimizing fewer parameters further reduces the model complexity and the risk of overfitting. Following these approaches, we regularize the training process by limiting the number of weights that can be modified at each training iteration. To identify the subset of weights most relevant to our optimization goal, we turn back to latent-space editing techniques, and specifically StyleCLIP. 

Recall that editing techniques aim to find directions in the latent space of a GAN that correspond to a change in a single attribute, and at the same time avoid unrelated changes. 
In the case of StyleGAN, it has been shown that the codes provided to different network layers can influence different semantic attributes. Thus, by considering editing directions in the \wplus space \cite{abdal2019image2stylegan} -- the latent space where each layer of StyleGAN can be provided with a different code $w_{i} \in \mathcal{W}$ -- we can identify which layers are most strongly tied to a given change. While we are interested in changes that cannot be achieved through mere latent code interpolations, we can still consider such editing directions locally (\ie at each iteration along the optimization process) and ask: `given the current version of the model, which layers are most relevant to our change?'. 

Building upon this intuition, we suggest a training scheme, where at each iteration we (i) select the $k$-most relevant layers, and (ii) perform a single training iteration of the generator to optimize only these layers, while freezing all the others. 
To select the $k$ layers,  
we randomly sample $N_{w}$ latent codes $\in \mathcal{W}$ and convert them to \wplus by replicating the same code for each layer. We then perform $N_{i}$ iterations of the StyleCLIP latent optimization step, with the current version of the generator held constant and using the global clip loss (\cref{eq:global_loss}). We select the $k$ layers for which the latent code changed most significantly. 
The two-step process is illustrated in \cref{fig:layer_focus}.

In all cases we additionally freeze StyleGAN's mapping network, affine code transformations, and all toRGB layers.

\input{resources/figures/layer_focus}

\input{resources/figures/generation_ffhq_small}

\subsection{Latent-Mapper `Mining'}\label{subsec:mapper}

\rgc{convert to paragraph instead of subsection}

\rev{As a last step, we note that for some shape changes, the generator does not undergo a complete transformation. In the case of dogs to cats, for example, the fine-tuning process results in a new generator that can output both cats, dogs, and an assortment of images that lie in between. Consider, however, that this shifted generator now includes \textit{both} cats and dogs within its domain. As such, we can now turn to standard editing techniques, and in particular StyleCLIP's latent mapper, in order to map all latent codes into the cat-like region of the latent space. We use the same network and training scheme as StyleCLIP, with the addition of the embedding-norm loss of Eq. \ref{eq:norm_loss}.}

